The $Z$-Curve as an $n$-Dimensional Hypersphere: Properties and Analysis

In this research, we introduce an algorithm that produces what appears to be a new mathematical object as a consequence of projecting the \( n \)-dimensional \( Z \)-curve onto an \( n \)-dimensional sphere. The first part presents the algorithm that enables this transformation, and the second part focuses on studying its properties.

==> changes.tex <==
\begin{document}
\section{Equivalent Position and the Minimum Number of Knowable Subsets}

Estimating the number of subsets of different sizes within a set \( \mathbf{X}^D_K \) using only the parameters \( D \) and \( K \) is challenging. Specifically, we cannot predict whether there are \( n \) subsets of size \( 2^D \times A \) or \( m \) subsets of size \( 2^D \times B \) after applying the circular projection to the set \( \mathbf{X}^D_K \).\\

However, we observe that \textit{certain regions in the $Z$-curve, when projected onto an $n$-dimensional sphere, consistently form subsets with the same number of elements}, even after subdividing each cell into \( 2^D \) smaller cells \( K \) times, regardless of the numerical values within each cell. A prominent example is the values located at the corners of the $Z$-curve, which always include zero. Independently of the value of \( K \), these regions consistently constitute a subset with exactly \( 2^D \) elements.\\

This suggests that when a parent cell divides into \( 2^D \) new child cells, one of them will always preserve its equivalent position, maintaining a subset size consistent with its parent. Therefore, for a given \( D \) and \( K \), knowing that the sum of all elements in subsets with the same number of elements remains constant (i.e., equal to \( \Psi \) or a multiple of it), the sum of the elements in the equivalent positions of \( \mathbb{T} \) will also yield a constant value associated with \( D \) and \( K + n \).

Consequently, we hypothesize the following:

\begin{conjecture}
\label{conj:min_subsets}
For given values of \( D \) and \( K = n + 1 \), the minimum number of subsets of different sizes in \( \mathbf{X}^D_K \) is at least equal to the number of subsets of different sizes when \( K = n \).
\end{conjecture}

This implies that when a cell divides into \( 2^D \) new cells, the \( 2^D - 1 \) cells that do not represent equivalent positions introduce uncertainty in how they will be grouped. To validate this conjecture, we can check whether the sum of the elements in the equivalent position subset equals the constant associated with the pair \( D \) and \( K \) using Equation \ref{eq:total_sum}. If it does, we confirm that it is a valid subset.\\

To calculate the equivalent position of a number in \( \mathbf{X}^D_S \) and map it to its corresponding position in \( \mathbf{X}^D_B \), where \( S \) (small \( K \)) is the scaling factor of the source and \( B = K + n \) (big \( K \)) is the scaling factor of the destination, we introduce the following function:

\begin{equation}
\phi(x) = 2^{D(B - S + 1)} \cdot \left\lfloor \frac{x}{2^D} \right\rfloor + \Omega \cdot (x \bmod 2^D),
\label{eq:position_eq}
\end{equation}

where \( \Omega \) is a constant with a binary representation given by:

\[
\Omega = \underbrace{(00\cdots 0)1}_{ D-1 \text{ zeros followed by a 1}} \text{ repeated } (B - S + 1) \text{ times}.
\]

This constant \( \Omega \) can be interpreted as a number whose binary form consists of a pattern of \( D - 1 \) zeros followed by a 1, repeated \( B - S + 1 \) times.

\begin{table}[H]
\centering
\caption{Values of $\Omega$ for $(B - S) \in \{1, 2, 3, 4\}$ across dimensions \( D \in \{1, 2, 3\} \).}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
B-S & \multicolumn{2}{c|}{Dimension = 1} & \multicolumn{2}{c|}{Dimension = 2} & \multicolumn{2}{c|}{Dimension = 3} \\ \hline
 & Binary & Decimal & Binary & Decimal & Binary & Decimal \\ \hline
% Row 1
1 & 11 & 3 & 0101 & 5 & 001001 & 9 \\ \hline
% Row 2
2 & 111 & 7 & 010101 & 21 & 001001001 & 73 \\ \hline
% Row 3
3 & 1111 & 15 & 01010101 & 85 & 001001001001 & 585 \\ \hline
% Row 4
4 & 11111 & 31 & 0101010101 & 341 & 001001001001001 & 4681 \\ \hline
% Row ....
5 & ... & ... & ... & ... & ... & ... \\ \hline
\end{tabular}
\label{your_label}
\end{table}

\textbf{Example 1:} Given the set of numbers \( \mathbf{X}^1_3 \), we wish to calculate their equivalent positions in \( \mathbf{X}^1_8 \). Using Equation \ref{eq:position_eq}, we have:

\[
\phi(x) = 2^{1(8 - 3 + 1)} \cdot \left\lfloor \frac{x}{2^1} \right\rfloor + 63 \cdot (x \bmod 2^1),
\]

where \( \Omega = 63 \) (since \( D = 1 \) and \( B - S + 1 = 6 \), and \( \Omega \) in binary is six repetitions of '1'). Simplifying:

\[
\phi(x) = 64 \cdot \left\lfloor \frac{x}{2} \right\rfloor + 63 \cdot (x \bmod 2).
\]

\begin{table}[H]
\centering
\caption{Equivalent positions of all \( n \in \mathbf{X}^1_3 \) in \( \mathbf{X}^1_8 \).}
\begin{tabular}{|c|cccccccc|}
\hline
\textbf{\( \mathbf{X}^1_3 \) Values} & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 \\
\hline
\textbf{Equivalent in \( \mathbf{X}^1_8 \)} & 0 & 63 & 64 & 127 & 128 & 191 & 192 & 255 \\
\hline
\end{tabular}
\end{table}

\textbf{Example 2:} For the set \( \mathbf{X}^2_2 \), we calculate their equivalent positions in \( \mathbf{X}^2_4 \):

\[
\phi(x) = 2^{2(4 - 2 + 1)} \cdot \left\lfloor \frac{x}{2^2} \right\rfloor + 21 \cdot (x \bmod 4),
\]

where \( \Omega = 21 \) (binary '010101'). Simplifying:

\[
\phi(x) = 64 \cdot \left\lfloor \frac{x}{4} \right\rfloor + 21 \cdot (x \bmod 4).
\]

\begin{table}[H]
    \caption{Equivalent positions of all \( n \in \mathbf{X}^2_2 \) in \( \mathbf{X}^2_4 \).}

    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
    \hline
    $\mathbf{X}^2_2$ Values & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 \\ \hline
    Equivalent in $\mathbf{X}^2_4$ & 0 & 21 & 42 & 63 & 64 & 85 & 106 & 127 \\ \hline
    \hline
    $\mathbf{X}^2_2$ Values & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\ \hline
    Equivalent in $\mathbf{X}^2_4$ & 128 & 149 & 170 & 191 & 192 & 213 & 234 & 255 \\ \hline
    \end{tabular}
    %\label{tab:my_label}
\end{table}


\begin{figure}[H]
\centering
\includegraphics[width=10cm]{Images/equiv_pos.png}
\caption{Left: Numbers in \( \mathbf{X}^2_2 \) arranged in a $Z$-pattern. Right: Equivalent positions in \( \mathbf{X}^2_4 \).}
\label{fig:equiv_positions}
\end{figure}

This function allows us to verify our initial hypothesis stated in Conjecture \ref{conj:min_subsets}. We demonstrate this through two examples, one in dimension three and another in dimension six.\\

\textbf{Example 3:} Consider the subset $ |\mathbb{T}|=16 \in \mathbf{X}^3_3$ with values $\{ $ 99, 327, 42, 270, 85, 369, 28, 312, 199, 483, 142, 426, 241, 469, 184, 412$\}$ we want to project them into their equivalent position in $\mathbf{X}^3_4$. The sum of all the elements in $\mathbb{T}$ is 4088, as dictates the Equation \ref{eq:total_sum} : 
\[
S(\mathbb{T}) = ( 2^{3(3+1)-1} - 2^{(3-1)} )\times \frac{16}{2^3} = 4088
\]


After we project the values of the given $\mathbb{T}\in\mathbf{X}^3_3$ into $\mathbf{X}^3_4$, we expect the sum of the projected values to be equal to 32760, which is the result from Equation \ref{eq:total_sum} for the parameters \( D = 3 \), \( K = 4 \) and $|\mathbb{T}|=16$.\\

The $\phi$ function given the parameters $B=4$, $S=3$ and $D=3$, $\Omega= 001001=9$, so $\phi$ will looks like : 
\[
\phi(\mathbb{T}) = 2^{3(4-3+1)} \cdot \left\lfloor \frac{x}{2^3} \right\rfloor + 9 \cdot (x \mod 2^3)
\]

Obtaining $\phi(\mathbb{T})=\mathbb{T'}=$ $\{ $795, 2623, 338, 2166, 685, 2953, 228, 2496, 1599, 3867, 1142, 3410, 1929, 3757, 1472, 3300$\}$. The result after summing all the new values is 32760, as we expected using Equation \ref{eq:total_sum}: 
\[
S(\mathbb{T'}) = ( 2^{3(4+1)-1} - 2^{(3-1)} )\times \frac{16}{2^3} = 32760
\]

\textbf{Example 4:} Consider the subset $|\mathbb{T}|=2816$ $\in \mathbf{X}^6_3$ with values listed in Appendix A, we want to project them into their equivalent positions in $\mathbf{X}^6_5$. The sum of all the values in $\mathbb{T}$ is 369097344, as dictates the Equation \ref{eq:total_sum} :

\[
S(\mathbb{T}) = ( 2^{6(3+1)-1} - 2^{(6-1)} )\times \frac{2816}{2^6} = 369097344
\]

After we project the values of the given $\mathbb{T}\in\mathbf{X}^6_3$ into $\mathbf{X}^6_5$, we expect the sum of the projected values to be equal to 1511828486784, which is the result from Equation \ref{eq:total_sum} for the parameters $D=6$, $K=5$ and $|\mathbb{T}|=2816$.\\

The $\phi$ function given the parameters $B=5$, $S=3$ and $D=6$, $\Omega=000001000001000001=4161$, so $\phi$ will looks like : 

\[
\phi(\mathbb{T}) = 2^{6(5-3+1)} \cdot \left\lfloor \frac{x}{2^6} \right\rfloor + 4161 \cdot (x \mod 2^6)
\]

The resulting values for $\phi(\mathbb{T})$, $\mathbb{T'}$, are provided in Appendix B. The total sum of the new vector of values is 1511828486784, which matches the expected result based on the Equation \ref{eq:total_sum}:


\[
S(\mathbb{T'}) = ( 2^{6(5+1)-1} - 2^{(6-1)} )\times \frac{2816}{2^6} = 1511828486784
\]

These examples support our conjecture by demonstrating that the minimum number of subsets of different sizes remains consistent or increases when moving from \( K = n \) to \( K = n + 1 \).
\end{document}
